On the Effectiveness of Virtual Reality-based Training for Robotic Setup

Virtual Reality (VR) is rapidly increasing in popularity as a teaching tool. It allows for the creation of a highly immersive, three-dimensional virtual environment intended to simulate real-life environments. With more robots saturating the industry - from manufacturing to healthcare, there is a need to train end-users on how to set up, operate, tear down, and troubleshoot the robot. Even though VR has become widely used in training surgeons on the psychomotor skills associated with operating the robot, little research has been done to see how the benefits of VR could translate to teaching the bedside staff, tasked with supporting the robot during the full end-to-end surgical procedure. We trained 30 participants on how to set up a robotic arm in an environment mimicking clinical setup. We divided these participants equally into 3 groups with one group trained with paper-based instructions, one with video-based instructions and one with VR-based instructions. We then compared and contrasted these three different training methods. VR and paper-based were highly favored training mediums over video-based. VR-trained participants achieved slightly higher fidelity of individual robotic joint angles, suggesting better comprehension of the spatial awareness skills necessary to achieve desired arm positioning. In addition, VR resulted in higher reproducibility of setup fidelity and more consistency in user confidence levels as compared to paper and video-based training.

==> excess_bib.tex <==
@article{fried2010virtual,
  title={From virtual reality to the operating room: the endoscopic sinus surgery simulator experiment},
  author={Fried, Marvin P and Sadoughi, Babak and Gibber, Marc J and Jacobs, Joseph B and Lebowitz, Richard A and Ross, Douglas A and Bent III, John P and Parikh, Sanjay R and Sasaki, Clarence T and Schaefer, Steven D},
  journal={Otolaryngology—Head and Neck Surgery},
  volume={142},
  number={2},
  pages={202--207},
  year={2010},
  publisher={SAGE Publications Sage CA: Los Angeles, CA}
}

@article{levin2018pre,
  title={Pre-course cognitive training using a smartphone application in orthopaedic intern surgical skills “boot camps”},
  author={Levin, Adam S and Haq, Ikram U and LaPorte, Dawn M},
  journal={Journal of orthopaedics},
  volume={15},
  number={2},
  pages={506--508},
  year={2018},
  publisher={Elsevier}
}

@article{broeders2019learning,
  title={Learning in the high-tech era: are we getting a grip on the learning curve?},
  author={Broeders, IAMJ},
  journal={Nederlands tijdschrift voor geneeskunde},
  volume={163},
  year={2019}
}

@article{edmond2002impact,
  title={Impact of the endoscopic sinus surgical simulator on operating room performance},
  author={Edmond Jr, Charles V},
  journal={The Laryngoscope},
  volume={112},
  number={7},
  pages={1148--1158},
  year={2002},
  publisher={Wiley Online Library}
}

@article{gallagher1999virtual,
  title={Virtual reality training in laparoscopic surgery: a preliminary assessment of minimally invasive surgical trainer virtual reality (MIST VR)},
  author={Gallagher, AG and McClure, N and McGuigan, J and Crothers, I and Browning, J},
  journal={Endoscopy},
  volume={31},
  number={04},
  pages={310--313},
  year={1999},
  publisher={Georg Thieme Verlag Stuttgart{\textperiodcentered} New York}
}

@article{aggarwal2007proving,
  title={Proving the effectiveness of virtual reality simulation for training in laparoscopic surgery},
  author={Aggarwal, Rajesh and Ward, Jonnie and Balasundaram, Indran and Sains, Parvinderpal and Athanasiou, Thanos and Darzi, Ara},
  journal={Annals of surgery},
  volume={246},
  number={5},
  pages={771--779},
  year={2007},
  publisher={LWW}
}

@article{pulijala2018effectiveness,
  title={Effectiveness of immersive virtual reality in surgical training—A randomized control trial},
  author={Pulijala, Yeshwanth and Ma, Minhua and Pears, Matthew and Peebles, David and Ayoub, Ashraf},
  journal={Journal of Oral and Maxillofacial Surgery},
  volume={76},
  number={5},
  pages={1065--1072},
  year={2018},
  publisher={Elsevier}
}

@incollection{higuchi2011robotic,
  title={Robotic instrumentation, personnel and operating room setup},
  author={Higuchi, Ty T and Gettman, Matthew T},
  booktitle={Atlas of Robotic Urologic Surgery},
  pages={15--30},
  year={2011},
  publisher={Springer}
}

@article{dewaele2019human,
  title={Is the Human Brain Capable of Controlling Seven Degrees of Freedom?},
  author={Dewaele, Frank and De Pauw, Tim and Kalmar, Alain and Pattyn, Piet and Van Herzeele, Isabelle and Mottrie, Alexandre and Van Nieuwenhove, Yves and Van Roost, Dirk},
  journal={Journal of Surgical Research},
  volume={238},
  pages={1--9},
  year={2019},
  publisher={Elsevier}
}

@article{amodeo2009robotic,
  title={Robotic laparoscopic surgery: cost and training.},
  author={Amodeo, A and Linares, A Quevedo and Joseph, JV and Belgrano, Emanuele and Patel, HR},
  journal={Minerva urologica e nefrologica= The Italian journal of urology and nephrology},
  volume={61},
  number={2},
  pages={121--128},
  year={2009}
}

@inproceedings{reiley2009task,
  title={Task versus subtask surgical skill evaluation of robotic minimally invasive surgery},
  author={Reiley, Carol E and Hager, Gregory D},
  booktitle={International conference on medical image computing and computer-assisted intervention},
  pages={435--442},
  year={2009},
  organization={Springer}
}



@article{ershad2019automatic,
  title={Automatic and near real-time stylistic behavior assessment in robotic surgery},
  author={Ershad, Marzieh and Rege, Robert and Fey, Ann Majewicz},
  journal={International journal of computer assisted radiology and surgery},
  volume={14},
  number={4},
  pages={635--643},
  year={2019},
  publisher={Springer}
}

@article{alarcon1996comparison,
  title={A comparison of operating room crowding between open and laparoscopic operations},
  author={Alarcon, A and Berguer, R},
  journal={Surgical endoscopy},
  volume={10},
  number={9},
  pages={916--919},
  year={1996},
  publisher={Springer}
}

@article{hortman2015positioning,
  title={Positioning considerations in robotic surgery},
  author={Hortman, Christina and Chung, Simon},
  journal={AORN journal},
  volume={102},
  number={4},
  pages={434--440},
  year={2015},
  publisher={Wiley Online Library}
}

